MAmmoTH: Building Math Generalist Models through Hybrid Instruction Tuning

We introduce MAmmoTH, a series of open-source large language models (LLMs) specifically tailored for general math problem-solving. The MAmmoTH models are trained on MathInstruct, our meticulously curated instruction tuning dataset. MathInstruct is compiled from 13 math datasets with intermediate rationales, six of which have rationales newly curated by us. It presents a unique hybrid of chain-of-thought (CoT) and program-of-thought (PoT) rationales, and also ensures extensive coverage of diverse fields in math. The hybrid of CoT and PoT not only unleashes the potential of tool use but also allows different thought processes for different math problems. As a result, the MAmmoTH series substantially outperform existing open-source models on nine mathematical reasoning datasets across all scales with an average accuracy gain between 16% and 32%. Remarkably, our MAmmoTH-7B model reaches 33% on MATH (a competition-level dataset), which exceeds the best open-source 7B model (WizardMath) by 23%, and the MAmmoTH-34B model achieves 44% accuracy on MATH, even surpassing GPT-4's CoT result. Our work underscores the importance of diverse problem coverage and the use of hybrid rationales in developing superior math generalist models.

==> achive.tex <==


% \begin{table}[t!]
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{lccccccccc|c}
% \toprule
% Training Data       & GSM8K                          & MATH                         & AQuA                         & NumGLUE                      & SVAMP                        & Mathematics                  & SimulEq                      & SAT                          & MMLU-M                    & AVG                          \\ \midrule
% \dataset             & 51.5                         & 28.5                         & 41.3                         & 53.9                         & 69                           & 45                           & 44.5                         & 35.4                         & 36.3                         & 45.0                         \\\midrule
% - Camel             & \cellcolor[HTML]{FCD2CA}52.4 & \cellcolor[HTML]{FCD8D0}28.8 & \cellcolor[HTML]{AED9F9}39.4 & \cellcolor[HTML]{B0DAF9}52.8 & \cellcolor[HTML]{A8D6F9}64.9 & \cellcolor[HTML]{AAD7F9}41.5 & \cellcolor[HTML]{ACD8F9}41.9 & \cellcolor[HTML]{B1DAF9}34.5 & \cellcolor[HTML]{FAAEA1}40.9 & \cellcolor[HTML]{B1DAF9}-0.9 \\
% - MATH              & \cellcolor[HTML]{ADD9F9}49.3 & \cellcolor[HTML]{99CFF8}19.1 & \cellcolor[HTML]{FBC3B9}43.7 & \cellcolor[HTML]{ADD9F9}51.7 & \cellcolor[HTML]{B0DAF9}67.7 & \cellcolor[HTML]{92CCF7}33.1 & \cellcolor[HTML]{FCCFC6}45.7 & \cellcolor[HTML]{FBC0B5}38.2 & \cellcolor[HTML]{FBC8BF}38.2 & \cellcolor[HTML]{AED9F9}-2.0 \\
% - AQuA              & \cellcolor[HTML]{B2DBF9}50.9 & \cellcolor[HTML]{B2DBF9}27.9 & \cellcolor[HTML]{80C4F6}23.2 & \cellcolor[HTML]{F9A799}59.2 & \cellcolor[HTML]{ACD8F9}66.2 & \cellcolor[HTML]{AED9F9}43.2 & \cellcolor[HTML]{AAD7F9}41.1 & \cellcolor[HTML]{A6D5F9}30.5 & \cellcolor[HTML]{9DD1F8}28.5 & \cellcolor[HTML]{A9D6F9}-3.8 \\
% - GSM8K               & \cellcolor[HTML]{6BBAF5}26.1 & \cellcolor[HTML]{B2DBF9}27.8 & \cellcolor[HTML]{ABD7F9}38.2 & \cellcolor[HTML]{B0DAF9}52.7 & \cellcolor[HTML]{96CEF8}58.8 & \cellcolor[HTML]{B2DBF9}44.5 & \cellcolor[HTML]{AAD7F9}41.2 & \cellcolor[HTML]{FCD6CE}35.9 & \cellcolor[HTML]{FBBEB2}39.3 & \cellcolor[HTML]{A7D6F9}-4.5 \\
% - MATH - AQuA       & \cellcolor[HTML]{AAD7F9}48.1 & \cellcolor[HTML]{94CDF7}17.4 & \cellcolor[HTML]{7FC3F6}22.8 & \cellcolor[HTML]{F78D7B}61.9 & \cellcolor[HTML]{AED9F9}67.2 & \cellcolor[HTML]{87C7F6}29.3 & \cellcolor[HTML]{B3DBF9}44.2 & \cellcolor[HTML]{9FD2F8}28.3 & \cellcolor[HTML]{9BD0F8}27.8 & \cellcolor[HTML]{A1D3F8}-6.4 \\
% - GSM8K - MATH        & \cellcolor[HTML]{5DB3F4}21.0   & \cellcolor[HTML]{99CFF8}19.2 & \cellcolor[HTML]{B1DAF9}40.5 & \cellcolor[HTML]{ACD8F9}51.2 & \cellcolor[HTML]{98CFF8}59.4 & \cellcolor[HTML]{90CBF7}32.7 & \cellcolor[HTML]{ABD8F9}41.6 & \cellcolor[HTML]{FCCDC4}36.8 & \cellcolor[HTML]{FCCCC3}37.8 & \cellcolor[HTML]{9FD2F8}-7.2 \\
% - GSM8K - MATH - AQuA & \cellcolor[HTML]{4EADF3}15.7 & \cellcolor[HTML]{91CBF7}16.3 & \cellcolor[HTML]{75BEF5}19.2 & \cellcolor[HTML]{F9A191}59.9 & \cellcolor[HTML]{99CFF8}59.7 & \cellcolor[HTML]{7EC3F6}26.2 & \cellcolor[HTML]{A2D4F8}38.5 & \cellcolor[HTML]{93CDF7}24.1 & \cellcolor[HTML]{9CD0F8}27.9 & \cellcolor[HTML]{8ECAF7}-14.1 \\ 
% \bottomrule
% \end{tabular}%
% }
% \caption{Influence of different major subsets in \dataset based on Llama-2 7B. Cells are blue if the
% removal hurts the performance compared with the full dataset, and orange if the removal boosts the performance.}
% \label{tab:ablation_dataset}
% \end{table}

